Universality of Cherenkov Light in EAS

The reconstruction of cosmic-ray-induced extensive air showers with a non-imaging Cherenkov detector array requires knowledge of the Cherenkov yield of any given air shower for a given set of shower parameters. Although air showers develop in a stochastic cascade, certain characteristics of the particles in the shower have been shown to come from universal probability distributions, a property known as shower universality. Both the energy and the angular distributions of charged particles within a shower have been parameterized. One can use these distributions to calculate the Cherenkov photon yield as an angular distribution from the Cherenkov cones of charged particles at various stages of shower development. This Cherenkov photon yield can then be tabulated for use in the reconstruction of air showers. In this work, we develop the calculation of both the Cherenkov angular distribution and Cherenkov yield per shower particle, and show how a look-up table was constructed to capture the relevant features of these distributions for general use. We compare the results of our calculations with the results of full, particle-stack, Monte Carlo simulation of the Cherenkov light produced in extensive air showers using CORSIKA-IACT. We make comparisons of both the lateral distribution of the Cherenkov photon flux amongst several detectors and of the arrival-time distribution of the Cherenkov photons in a single detector.

==> lateral.tex <==
\section{Lateral Distribution}
As EAS develop, they spread out in space. To first order, the source locations of Cherenkov light in an EAS can be assigned to points along the shower axis. For Cherenkov telescopes far away from the axis, this approximation is sufficient. However, in the regime where the distance between the shower axis and the counter location is similar to the lateral spread of the shower itself, it is necessary to spread the Cherenkov production vectors away from the shower axis. The universality of shower width has been established in the domain of dimensionless Moliere units $X$, to account for shower development in various atmospheric densities, and has been parameterized by several groups \cite{Lafebre} \cite{NKG}. 

\begin{equation}
    X = \frac{r}{r_m}
\end{equation}

\begin{equation}
    r_m \approx \frac{96 } {\rho(h) } \frac{kg/m^2}{kg/m^3}
\end{equation}

For this study, it is sufficient to use the energy independent lateral distribution parameterized by \cite{NKG}. This distribution is normalized over all log Moliere units $l_x = \ln{X}$ \cite{Lafebre}.

\begin{equation}
  G_M(t,l_X) = \frac{\partial N_e}{\partial l_X} = C_0 X^{\zeta_0}(X_1+X)^{\zeta_1}
\end{equation}

To find the relative density of particles per unit area we perform two changes of variables. First from the $l_X$ domain to $X$.

\begin{eqnarray}
  \frac{\partial N_e}{\partial X} &=& \frac{\partial N_e}{\partial l_X} \frac{\partial l_X}{\partial X}\\
                        &=& \frac{\partial N_e}{\partial l_X} \frac{1}{X}
\end{eqnarray}

Now we convert to density of particles per unit area.

\begin{eqnarray}
  \frac{\partial N_e}{\partial r} &=& \frac{\partial N_e}{\partial X} \frac{\partial X}{\partial r}\\
                        &=& \frac{\partial N_e}{\partial X} \frac{1}{r_m}
\end{eqnarray}

\begin{eqnarray}
  \frac{\partial N_e}{\partial A} &=& \frac{\partial N_e}{\partial r} \frac{1}{2 \pi r}\\
                        &=& \frac{\partial N_e}{\partial r} \frac{1}{2 \pi X r_m}\\
                        &=& \frac{\partial N_e}{\partial l_X} \frac{1}{2 \pi X^2 r_m^2}\\
\end{eqnarray}

To find the average distance from the shower axis, we integrate $\frac{\partial N_e}{\partial A}$ over all area in the shower cross section for a given stage $t$ and Moliere radius $r_m(h)$.

\begin{eqnarray}
    \overline{r} &=& 2 \pi \int_0^\infty \ud r \; r^2 \frac{\partial N_e}{\partial A} \\
                 &=& \int_0^\infty \ud r \; \frac{\partial N_e}{\partial l_X}
\end{eqnarray}

where $l_X(r,r_m) = \ln{X} = \ln{\frac{r}{r_m}}$. Converting back to Moliere units so this average can be used independently of atmospheric density:

\begin{equation}
    \frac{\partial N_e}{\partial A_X} = \frac{\partial N_e}{\partial X} \frac{1}{2 \pi X} = \frac{\partial N_e}{\partial l_X} \frac{1}{2 \pi X^2}
\end{equation}

\begin{eqnarray}
    \overline{X} &=& 2 \pi \int_0^\infty \ud X \; X^2 \frac{\partial N_e}{\partial A_x} \\
                 &=& \int_0^\infty \ud X \; \frac{\partial N_e}{\partial l_X}
\end{eqnarray}

==> table.tex <==
\section{Tabulation of Cherenkov Distributions}
To simulate the Cherenkov signal of an extensive air shower, we need Cherenkov angular distributions corresponding to all possible shower development stages at all possible altitudes in the atmosphere. 
